Theoretical Guarantees for the Statistical Finite Element Method

The statistical finite element method (StatFEM) is an emerging probabilistic method that allows observations of a physical system to be synthesised with the numerical solution of a PDE intended to describe it in a coherent statistical framework, to compensate for model error. This work presents a new theoretical analysis of the statistical finite element method demonstrating that it has similar convergence properties to the finite element method on which it is based. Our results constitute a bound on the Wasserstein-2 distance between the ideal prior and posterior and the StatFEM approximation thereof, and show that this distance converges at the same mesh-dependent rate as finite element solutions converge to the true solution. Several numerical examples are presented to demonstrate our theory, including an example which test the robustness of StatFEM when extended to nonlinear quantities of interest.

==> paper_material/experiment_impl_details.tex <==
%!TEX root=../ex_supplement.tex

\begin{remark}\label{rem:cov_loading_approx}
    In both the \ac{statfem} prior and posterior the $n_u\times n_u$ matrix $K_{\mathcal{F}_{h}}=\mathcal{F}_{h}K\mathcal{F}_{h}^{\dagger}$ appears. This is the covariance matrix for the random load vector $\mathbf{f}=\mathcal{F}_{h}f$. The $ij$\textit{-th} element of this covariance matrix is given by:
    \begin{equation}\label{eq:load_vect_cov_mat_entries}
        (K_{\mathcal{F}_{h}})_{ij}=\int_{D}\int_{D}\phi_{i}(x)k_{f}(x,y)\phi_{j}(y)\mathrm{d}x\mathrm{d}y .
    \end{equation}
    For a covariance function $k_f$ which is globally supported, the covariance matrix, $K_{\mathcal{F}_{h}}$, is dense as can be seen from expression \cref{eq:load_vect_cov_mat_entries} above. As such, it can be very difficult to efficiently compute and assemble the entries of this matrix. We thus employ an approximation of this matrix, by interpolating the covariance function $k_f$ with the finite element basis functions, as suggested by \cite{Girolami2021}. I.e., denoting the non-boundary nodes of the FE triangulation by $\left\{ x_{i} \right\}_{i=1}^{n_u}$, we approximate $k_f$ by,
    \begin{equation}\label{eq:k_f_approx}
        k_f(x,y) \approx\sum_{k,l=1}^{n_u}\phi_{k}(x)k_{f}(x_{k},x_{l})\phi_{l}(y)
    \end{equation}
    Using this interpolation of $k_f$ we can approximate the entries of $K_{\mathcal{F}_{h}}$ by,
    \begin{align*}
        (K_{\mathcal{F}_{h}})_{ij} &\approx \sum_{k,l=1}^{n_u}k_{f}(x_{k},x_{l})\int_{D}\int_{D}\phi_{i}(x)\phi_{k}(x)\phi_{j}(y)\phi_{l}(y)\mathrm{d}x\mathrm{d}y \\
        &= \sum_{k,l=1}^{n_u}k_{f}(x_k,x_l)\int_{D}\phi_i(x)\phi_{k}(x)\mathrm{d}x\int_{D}\phi_j(y)\phi_{l}(y)\mathrm{d}y \\
        &= \sum_{k,l=1}^{n_u}k_{f}(x_k,x_l)M_{ik}M_{jl} \\
        &= (MC_{f}M^{T})_{ij}
    \end{align*}
    i.e.\ we can approximate:
    \begin{equation}
        K_{\mathcal{F}_{h}}\approx MC_{f}M^{T}
    \end{equation}
    where $C_f\in\R^{n_{u}\times n_{u}}$ is the covariance matrix corresponding to evaluating $k_{f}$ on the non-boundary nodes, $\left\{ x_{i} \right\}_{i=1}^{n_u}$, of the \ac{fem} triangulation, and $M$ is the mass matrix introduced in \cref{main-sec:fem}. This approximation will improve as $h$ gets smaller. \mylozenge
\end{remark}
\begin{remark}\label{rem:approx_for_cov_cont_wasser}
    Since all of the true and \ac{statfem} priors and posteriors are Gaussian measures, and since we are interested in demonstrating a bound on the error between the respective priors and posteriors for the Wasserstein-2 distance the expression \cref{main-eq:wasser_for_gaussians} will be useful. 
    Focussing on the covariance contribution in \cref{main-eq:wasser_for_gaussians}, note that this is difficult to compute explicitly for the measures in this paper.
    For two \acp{gp} $\nu_i \sim \mathcal{N}(0, \Sigma_i)$, $i\in\{1,2\}$ we approximate the covariance contribution by fixing a fine reference grid $\left\{ \tilde{x}_{i} \right\}_{i=1}^{N}$, computing the covariance matrices, $C_{i}=\left\{ k_{i}(\tilde{x}_{k},\tilde{x}_{l}) \right\}_{k,l=1}^{N}$, corresponding to the covariance operators, $\Sigma_{i}$, evaluated on this reference grid, where $k_{i}$ is the covariance function associated with $\Sigma_{i}$ respectively, and finally approximating the Wasserstein distance as follows:
    \begin{align}
        W^{2}(\mathcal{N}(0,\Sigma_{1}),\mathcal{N}(0,\Sigma_{2}))&=\tr(\Sigma_{1})+\tr(\Sigma_{2})-2\tr\sqrt{\Sigma_{1}^{1/2}\Sigma_{2}\Sigma_{1}^{1/2}}\nonumber \\
        &\approx\tr(C_{1})+\tr(C_{2})-2\tr\sqrt{C_{1}^{1/2}C_{2}C_{1}^{1/2}}.
    \end{align}
    \mylozenge
\end{remark}
\begin{remark}\label{rem:mean_cont_wasser}
    Let $m_{\star},m_{h}$ denote the means of the true and \ac{statfem} prior (or posterior) respectively. The mean contribution to the Wasserstein-2 distance is $\|m_{\star}-m_{h}\|_{L^{2}(D)}$. This contribution can be easily approximated by utilising a modern \ac{fem} package such as \texttt{FEniCS}, which we use in this paper. \mylozenge
\end{remark}
